Memory-based Deep Reinforcement Learning for Obstacle Avoidance in UAV with Limited Environment Knowledge

This paper presents our method for enabling a UAV quadrotor, equipped with a monocular camera, to autonomously avoid collisions with obstacles in unstructured and unknown indoor environments. When compared to obstacle avoidance in ground vehicular robots, UAV navigation brings in additional challenges because the UAV motion is no more constrained to a well-defined indoor ground or street environment. Horizontal structures in indoor and outdoor environments like decorative items, furnishings, ceiling fans, sign-boards, tree branches etc., also become relevant obstacles unlike those for ground vehicular robots. Thus, methods of obstacle avoidance developed for ground robots are clearly inadequate for UAV navigation. Current control methods using monocular images for UAV obstacle avoidance are heavily dependent on environment information. These controllers do not fully retain and utilize the extensively available information about the ambient environment for decision making. We propose a deep reinforcement learning based method for UAV obstacle avoidance (OA) and autonomous exploration which is capable of doing exactly the same. The crucial idea in our method is the concept of partial observability and how UAVs can retain relevant information about the environment structure to make better future navigation decisions. Our OA technique uses recurrent neural networks with temporal attention and provides better results compared to prior works in terms of distance covered during navigation without collisions. In addition, our technique has a high inference rate (a key factor in robotic applications) and is energy-efficient as it minimizes oscillatory motion of UAV and reduces power wastage.

==> darqn-plot.tex <==
% \begin{tikzpicture}[scale=0.5]
% \begin{axis}[]
% \addplot [color=blue, only marks, mark=o,]
%  plot [error bars/.cd, y dir = both, y explicit]
%  table[x =x, y =y, y error =ey]{dataerror.csv};
%  \end{axis}
% \end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[]
\addplot [color=blue, only marks,mark=o,]
 plot [error bars/.cd, y dir = both, y explicit]
 table[row sep=crcr, x index=0, y index=1, x error index=2, y error index=3,]{
12 4 3.385995 0.866002\\
11 2 3.133745 0.937226\\
9 9 2.906316 0.895013\\
8 7 2.586054 0.835342\\
7 4 2.346789 0.792954\\
6 1 2.283117 0.699818\\
4 9 2.012212 0.909995\\
3 7 1.919941 1.366541\\
2 4 1.809623 1.691634\\
1 1 5.603446 13.825383\\
};
\end{axis}
\end{tikzpicture}%

==> impl.tex <==
\subsection{Model and Simulation Settings}
For RL algorithms to learn an effective collision avoidance policy, the UAV learning agent must have enough experience of undesirable events like collision. Training learning algorithms on a fragile drone in a physical environment is expensive and hence the performance of DRL algorithms is usually demonstrated on simulated environments. In this work, we build and test our UAV collision avoidance algorithms on a variety of simulated environments (built on Gazebo\footnote{\href{www.gazebosim.org}{www.gazebosim.org}} simulator), each of which has different characteristics. Some of the environment snapshots are shown in Fig. \ref{fig:collage}. 
\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.06]{collage_ppr}
  \caption{\small Screenshots of the designed environments in Gazebo. We cover a large range of colors, textures, sizes and shapes for obstacles and walls.}
  \label{fig:collage}
\end{center}
\end{figure}
We have a total of 22 different simulated indoor environments, of which few are inspired from \cite{punarjay} and rest are self designed. The environments consist of broad and narrow hallways, small and large enclosed areas with structured and unstructured obstacles like humans, traffic cones, tables etc and floors ranging from asphalt to artificial turf. The walls and obstacles with a wide range of shape, texture and color provide highly diversified visual information for effective learning.
\textbf{In Gazebo simulator, the observation from the environment needs to be simulated}. \textbf{For this, Kinect sensor for the drone in simulator was used.} Henceforth, we refer to these image pairs as RGB-D image pairs. \textbf{In order to ensure that the policy learnt in simulation generalizes well to real-world scenarios, we opted to add noise to the RGB images used for finding depth maps.
These RGB images were degraded with Gaussian blurring, random jitter and superpixel replace with replacement probability 0.5.}

Our method initially trains the UAV by starting off with simple hallway environments free of obstacles. Gradually the environment complexity is increased by narrowing down the pathway and eventually training in an enclosed space with densely placed obstacles. The \textbf{DARQN} network is trained to learn the observation-action value over the last $L$ observations (depth images received from the simulated Kinect sensor) corresponding to the three actions \emph{``go straight"}, \emph{``turn left"} and \emph{``turn right"}.  The agent receives a reward after each step and \textbf{this reward function is defined as}
$$R_i=\min\bigg(1,\frac{d_i - r_{drone}}{\sigma - r_{drone}}\bigg)$$ 
where $d_i$ is the nearest pixel distance at $i^{th}$ step, $\sigma$ is the threshold distance and $r_{drone}$ is the radius of the drone. If the agent collides, the episode ends with a penalty of -10. Otherwise, the episode lasts until it reaches the maximum number of steps (1000 steps) and terminates with no penalty. The agent also receives additional +0.5 reward if it chooses the ``go straight" action. The reward is designed to let agent prefer move forward action at empty places and takes turns near the obstacles.
\textbf{we need to explain more that for energy efficiency or lesser time goals we have designed reward function to go straight always and no reward for turning. also, if there's no obstacle in the way it will simply go straight and only turns on perceiving an obstacle}
To cope with the issue of exploration-exploitation a linear annealed policy is utilized during training with initial $\epsilon$ = 1 dropping to 0.05 as the final value. The network hyper-parameter values are as shown in Table \ref{hyperparam}. 
\begin{table}
\begin{center}
\begin{tabular}{ c | c }
  Entity & Value  \\
  \hline
  Discount Factor ($\gamma$) & 0.99  \\
  Mini-batch size & 32  \\
  Learning rate & 0.0001  \\
  Target network update frequency & 400 \\
  Input observation size & 84$\times$84 \\
  Conv1 layer filter size & 8$\times$8 \\
  Conv2 layer filter size & 4$\times$4 \\
  Conv3 layer filter size & 3$\times$3 \\
\end{tabular}
\caption{\small Hyperparameter values of proposed control network}
\label{hyperparam}
\end{center}
\end{table}


% For effective obstacle avoidance in real-world scenarios, the learned policy in simulation needs to be generalizable. However, this is highly challenging because of the huge gap in visual information available in the real and simulated worlds. Moreover, the depth maps produced by the proposed depth network are too noisy when compared to depth images obtained from the simulated kinect sensor. To overcome this, we degraded the sensor images with Gaussian blurring, random jitter and superpixel replace with replacement probability 0.5. This is crucial for non-linear function approximators to learn and generalize well and thus become transferable to real-world systems.


\subsection{Depth Network Settings}
 The proposed Conditional GAN is initially trained on a total of $90000$ RGB-D image pairs collected from the Gazebo simulated environments. The image pairs were collected by using a Kinect sensor mounted on the flying drone in simulation, covering all possible viewpoints. Further, the data is augmented off-line by random flipping, adding random jitter and random alteration to the brightness, saturation, contrast and sharpness. The network is trained on the entire collected data for $20$ epochs in batch size of $4$ on an NVIDIA Titan X machine. The network is fine-tuned using $8000$ and $16000$ augmented pairs from RGBD-human-explore data \cite{ram-lab} and NYU2 dataset \cite{nyu2} respectively.




% \subsection{Control Network}
% For reinforcement learning algorithms to learn an effective collision avoidance model, the agent must have enough experience of undesirable events like collision. Training learning algorithms on a fragile drone in a physical environment is expensive and avoided. To overcome this, we use simulated training environments, providing ample experience data which otherwise would be laborious to collect from demonstration method. We utilized the above mentioned simulated environments and started training in a simple, broad hallway environment with no obstacle. 
% The network is trained to predict the state-action value over the last $L$ observations (depth images received from the simulated Kinect sensor) corresponding to the three actions \emph{"go straight", "turn left" and "turn right"}; action with the highest Q-value is executed. Over the time, we increase the difficulty of the environment by narrowing down the pathway and eventually training in an enclosed space with densely placed obstacles. To cope with the issue of exploration-exploitation a linear annealed policy is utilized during training with initial $\epsilon$ = 1 dropping to 0.5 as the final value. Rest of the details on the network hyper-parameter values are shown in Table \ref{hyperparam} \par

% The agent receives a reward after each step, defined as- 
% $$R_i=\min\bigg(1,\frac{d_i - r_{drone}}{\sigma - r_{drone}}\bigg)$$ 
% where $d_i$ is the nearest pixel distance at $i^{th}$ step, $\sigma$ is the threshold distance and $r_{drone}$ is the radius of the drone. If the agent collides, the episode ends with a penalty of -10. Otherwise, the episode lasts until it reaches the maximum number of steps (1000 steps) and terminates with no punishment. The agent also receives additional +0.5 reward if it chooses the $"go forward"$ action. The reward is designed to let agent prefer move forward action at empty places and takes turns near the obstacles. \par

% In order to apply it in practice for robotic applications, the learned policy should be effectively transferable to the real-physical systems. However, this is highly challenging because of the huge gap in visual information available in the real and simulated worlds. Moreover, the depth maps produced by the proposed depth network are too noisy when compared to depth images obtained from the simulated kinect sensor. To overcome this, we degraded the sensor images with Gaussian blurring, random jitter and superpixel replace with replacement probability 0.5. This is crucial for non-linear function approximators to learn and generalize well and thus become transferable to real-world systems.




==> method.tex <==
The objective of our work is to find a suitable policy (a sequence of actions given states of the environment) for UAV navigation that avoids obstacles (both stationary and mobile). We propose a general method for this which can incorporate an overall path objective, such as defining start and goal positions. 

\subsection{Problem Definition}
In order to safely navigate without colliding against obstacles in an indoor or outdoor environment, the UAV needs to be aware of the state $s$ of the environment. 
The state of the environment is a tuple of properties of the environment which characterize it and aid the UAV in navigation. Once the state $s$ is known, the UAV selects an appropriate action $a$. The action the UAV chooses affects the state of the environment - in the obstacle avoidance problem, this means the UAV chooses to move in some particular direction leading to a change in its position and/or orientation. The UAV gets to observe more obstacles or perhaps more free space in front depending on this change in position and/or orientation. As noted in Section \ref{sec:intro}, the UAV needs to choose an action depending on the state at every instant $t$ when it navigates through the environment. Further, each action taken affects future states and hence future decisions of the UAV. Based on the action taken, the realization of the next state is probabilistic (and hence uncertain) implying that navigating by avoiding obstacles is a sequential decision making problem in the face of uncertainty.

Prior works \cite{cad2rl,arxivref2} assume that the monocular image of the environment is a good indicator of the state of the environment. However, since the UAV's monocular camera has a limited field of vision, we believe the UAV controller cannot infer the full state of the environment using the RGB image. Instead, the UAV controller only has an estimate of the state and this estimate is formally known as an \emph{observation}. In the method we propose, the inputs to our model consist of monocular RGB images without depth or other sensory inputs, whereas the \emph{observation} is the predicted depth map obtained from the monocular image. Based on these assumptions, we model the UAV obstacle avoidance and navigation problem in the framework of partially observable Markov decision processes (POMDPs).

We propose a POMDP model $\langle S,A,P,R,\Omega,\mathcal{O},\gamma \rangle$ for the obstacle avoidance problem. Here $S$ is the set of states of the environment, referred to as ``state space", while $A$ is the set of \emph{feasible} actions and referred to as the ``action space''. $P$ 
is the transition probability function that models the evolution of states based on actions chosen and is defined as $P: S\times A \times S\rightarrow [0,1]$. $R$ is the \emph{reinforcement} or the \emph{reward} function defined as $R: S \times A \rightarrow \R$. The reward function serves as a \emph{feedback} signal to the UAV for the action chosen. For instance, in a state $s$ if the UAV selects an action $a$ which steers it away from an obstacle, the reward for that state-action pair $(s,a)$ is positive, implying that the action $a$ is beneficial in the state $s$, while picking an action which results in collision will naturally yield a negative reward. $\Omega$ is the set of observations and an observation $o \in \Omega$ is an estimate of the true state $s$. $\mathcal{O}:S \times A \times \Omega \rightarrow [0,1]$ is a conditional probability distribution over $\Omega$, while $\gamma \in (0,1)$ is the discount factor. At each time $t$, the environment state is $s_t \in S$. The UAV takes an action $a_t \in A$ which causes the environment to transition to state $s_{t+1}$ with probability $P(s_{t+1}|s_t,a_t)$. Based on this transition the UAV receives an observation $o_t \in \Omega$ which depends on $s_{t+1}$ with probability $\mathcal{O}(o_t|s_{t+1},a_t)$. The aim is to solve the obstacle avoidance problem, which translates to the task of finding an optimal \emph{policy} $\pi^*:\Omega \rightarrow A $. By determining an optimal policy, the UAV controller is able to select an action at each time step $t$ that maximizes the expected sum of discounted rewards, which is defined as $\E \left[ \sum\limits_{t=0}^{\infty} \gamma^t R(s_t,a_t)\right]$. 
\subsection{Model}
We need to define the sets $\Omega$, $A$ and the functions $R,P,\mathcal{O}$ in order to find an optimal policy. 
The input to our model is the monocular RGB image, without any depth information. Our model extracts the depth map from the RGB image and this is the observation for the UAV controller. Such a depth map indicates the distance between the objects and the UAV. The feasible actions ($A$) available for the UAV given an observation are ``go straight'', ``turn right'' and ``turn left'', respectively. The reward function $R$ is designed using the depth information and its exact analytical form is explained in Section \ref{sec:exp}. In order to determine the functions $P$ and $\mathcal{O}$, we must be aware of the structure of environment and the motion dynamics of the UAV. In practice, these are impossible to know, since ultimately the UAV must be capable of navigating in unknown, unstructured environments in presence of other factors like wind, turbulence etc. Thus, we propose a Reinforcement learning technique to find an optimal policy for UAV navigation. Reinforcement learning is a model-free learning-based approach to solve POMDPs when the model information via $P$ and $\mathcal{O}$ is not available.

In order to learn a good policy, one of the approaches in RL is to learn the optimum Q-value of every observation-action $(o,a)$ pair using an iterative algorithm (similar to \cite{ql}). The Q-value $Q^\pi(o,a)$ is defined as the expected sum of discounted rewards obtained by taking the action $a$ upon observation $o$ and following the policy $\pi$ thereafter. The optimal Q-values are defined as 
$$
Q^*(o,a) = \max_{\pi} Q^\pi(o,a).
$$
Once the optimum Q-values of an observation $o$ are obtained, the optimal action is picked by finding $arg \max\limits_a Q(o,a)$. However, iteratively learning the Q-values requires maintaining and updating these values for all observation-action pairs. This turns out to be computationally infeasible. We present a memory augmented convolutional neural network architecture to approximate the Q-values using feature vectors. This is similar in spirit to DQN\cite{dqn} and DRQN \cite{drqn}. The performance of the proposed architecture for UAV obstacle avoidance is analyzed in Section \ref{sec:results}.

\subsection{Deep Recurrent Q-Network with Temporal Attention}
The architecture for approximating Q-values is based on deep recurrent Q-network with attention. This approach essentially keeps track of the past few observations. The recurrent network possesses the ability to learn temporal dependencies by using information from an arbitrarily long sequence of observations, while the temporal attention weighs each of the recent observations based on their importance in decision-making. 

At time $t$, the proposed model utilizes a sequence of recent $L$ observations ${o_{t-(L-1)},...,o_t}$. Each observation $o_{t-(L-i)}, \; 0 \leq i \leq L$, which is a depth map, is processed by convolutional layers of the network, followed by a fully connected layer augmented with LSTM \cite{lstm} recurrent network. The DRQN model with LSTM estimates $Q(o_t,h_{t-1},a_t)$, where $h_{t-1}$ is the hidden state of the controller and is determined 
 as $h_{t-1}=LSTM(h_{t-2},o_{t-1})$. The hidden state represents the information gathered over time. 
 
 \begin{figure}[t]
\begin{center}
\includegraphics[scale=0.4]{darqn_final}
\caption{\small Control Network: Architecture of Deep Recurrent Q-Network with Temporal Attention. Number of filters, stride and output size are mentioned for each convolutional layer.}
\label{fig:darqn}
\end{center}
\end{figure}
 
Following the LSTM layer, we propose the use of Temporal Attention \cite{temporal} in our model for evaluating the informativeness of each observation in the sequence. Temporal attention optimizes a weight vector with values depicting the importance of observations at the previous instants. This also increases the training speed and provides better generalizability over training data. Let $(\mathbf{v}_{t-(L-1)},\mathbf{v}_{t-(L-2)},\ldots,\mathbf{v}_t)^\top$ be the feature vectors obtained from the convolutional layers, over the past $L$ observations. Using the hidden states, the weight vector $(e_{t-(L-1)},e_{t-(L-2)},\ldots,e_{t})^\top$ over the $L$ feature vectors is computed using the $\tanh$ activation function:
\begin{equation}
e_{t-(L-i)} = \mathbf{w}^\top\tanh \left(W_ah_{t-1} + U_a \mathbf{v}_{t-(L-i)} + b_a\right)
\end{equation}
in which $\mathbf{w},b_a \in \R^a,W_a \in \R^{a\times r},U_a \in \R^{a \times m}$ are all learnable parameters and $h_t \in \R^r$. Here, we assume that $r$ is the size of an RNN hidden state, $m$ is the encoding size of CNN and $a$ as the attention matrix size. The $\tanh$ activation function is applied pointwise on the vector obtained from $W_ah_{t-1} + U_a \mathbf{v}_{t-(L-i)} + b_a$.

These weights are normalized using the softmax function
\begin{equation}
a_{t-(L-i)} = \frac{\exp(e_{t-(L-i)})}{\sum\limits_{j=1}^{L} \exp(e_{t-(L-j)})}.
\end{equation}
Further, to predict the Q-values a context vector is computed using the above calculated softmaxes and hidden states as:
$$\phi(t) = \sum\limits_{j=1}^{L} (a_{t-(L-j)} v_{t-(L-j)}). $$ Given the context vectors, the Q values of $(o,a)$ pairs are approximated by the ReLU activation functions which output the approximated Q-values. $Q(o,a) \approx Q(o,a,r) = f(p,\phi_1(t),\ldots,\phi_m(t))$, where $f$ is some non-linear function of the context vectors. In the above approximation, $p$ represents the weight vector. This vector is computed using experience replay and fixed Q-targets. 
An \emph{experience} is a collection of $(o,a,o',r)$ transition-reward tuples which are stored in memory. Mini-batches of transitions are sampled (i.e., replayed from memory) from this collection and used for update of the weight vector $p$, starting from some initial configuration. The loss function used to update the weight vector in $i^{th}$ iteration is given as:
$$L(p_i) = \E \left[ (r_i + \gamma \max\limits_a Q(o',a',p^-_i) - Q(o,a,p_i) )^2 \right],$$ where $p^-_i$ represents weights from the previous iteration. The loss function can be minimized by computing its gradient as follows:
\begin{equation*}
\begin{split}
\nabla_{p_i} L(p_i) = \E [ (r_i + \gamma \max\limits_a Q(o',a',p^-_i) -  Q(o,a,p_i) ) \\\nabla_{p_i}Q(o,a,p_i) ].
\end{split}
\end{equation*}
% The obtained context vector is input to a single fully connected layer with ReLU\cite{relu} activation functions that outputs approximated Q-value for each action. 
The complete model is trained by minimizing a loss function as described in \cite{drqn}. The proposed model using temporal attention is illustrated in Fig \ref{fig:darqn}.

\subsection{Obtaining depth maps from RGB images}
The UAV's on-board sensor is limited to providing monocular RGB image data. Effective depth prediction from an RGB image is essential when operating in the physical world. Learning a mapping for image translation $X\rightarrow Y$, given image pairs $\{x \in X,y \in Y\}$, is a challenging task in computer vision community. In this work, we propose the use of conditional generative adversarial network (cGAN) \cite{pix2pix} for this image-to-image translation. This approach uses two separate ConvNets (called as Generator and Discriminator) with BatchNorm layers and ReLU activation layers. The Generator (G) ConvNet is an encoder-decoder structure with skip connections, designed to generate realistic fake images taking $x\in X$ and a noise vector z as inputs. The Discriminator (D) network classifies randomly picked images as fake or real with a cross-entropy loss. Let $\theta_D$ and $\theta_G$ represent the parameters of the Discriminator and Generator networks respectively. The Generator is expected to produce images close to the ground truth, while the discriminator is supposed to distinguish fake images from the real images. Hence in a sense, the objectives of these two networks are opposed to each other. The loss function $\mathcal{L}_{cGAN}(\theta_G,\theta_D)$ defined below reflects these objectives:
\begin{equation}
\begin{split}
\label{discloss}
% \begin{aligned}
% \mathop{\mathbb{E}}_{x,y~p_{data(x,y)}} [\log(D(x,y))] +\cap \mathop{\mathbb{E}}_{x~p_{data(x), z~p_z(z)}} [\log(1-D(x,G(x,z)))]
\mathcal{L}_{cGAN}(\theta_G,\theta_D) = \mathbb{E}_{x,y \sim p_{data}} [\log D(x,y)] + \\
\mathbb{E}_{x\sim p_{data}(x), z \sim p_z(z)} [\log(1-D(x,G(x,z)))].
% \end{aligned}
\end{split}
\end{equation}
In the above equation, the variable $x$ is the RGB image and $y$ is its true depth map. The depth map generated by G is denoted as $G(x,z)$. $D(x,y)$ and $D(x,G(x,z))$ are the probabilities of the image belonging to the real class.
Training a cGAN involves a few steps. Initially, the discriminator is trained on real and fake depth images with the correct labels for few epochs. Following this, the generator is trained using the predictions from the trained discriminator as its objective. This procedure is repeated for few epochs until the generated fake depth maps are difficult to distinguish from the real depth maps. The cGAN architecture is illustrated in Fig.\ref{fig:pix2pix}. The approach also incorporates $L1$ loss to generate better near ground truth images.
\begin{equation}
\begin{split}
\label{l-one}
% \begin{aligned}
% \mathop{\mathbb{E}}_{x,y~p_{data(x,y)}} [\log(D(x,y))] +\cap \mathop{\mathbb{E}}_{x~p_{data(x), z~p_z(z)}} [\log(1-D(x,G(x,z)))]
\mathcal{L}_{L1}(\theta_G) = \mathbb{E}_{x,y \sim p_{data}, z \sim p_z(z)} [\lVert y-G(x,z) \rVert_1].
% \end{aligned}
\end{split}
\end{equation}
Hence the final objective of the model can be analytically represented as
\begin{equation}
\label{gan_loss}
\min_{\theta_G} \max_{\theta_D} \{\mathcal{L}_{cGAN} (\theta_G,\theta_D) + \lambda \mathcal{L}_{L1}(\theta_G)\},
\end{equation}
where $\lambda$ is an adjustable hyper-parameter. In contrast to previous methods (\cite{fcrn}-\cite{semisupdeeplearningdepth}) our approach learns a loss function adaptable to the input data making it domain independent and suitable for our problem of intermediate depth prediction for obstacle avoidance.


\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.25]{pix_final}
  \caption{\small Depth Network: Conditional GAN architecture}
  \label{fig:pix2pix}
\end{center}
\end{figure}

==> motivation.tex <==
Our work adds a new dimension to the existing work on UAV obstacle avoidance. We are motivated from how humans decide what to do next given a scenario. Humans have \emph{limited} or \emph{partial access} to the environment, but still are able to solve challenging problems in daily lives. All this is possible, because human brain has memory which is key to summarizing and storing relevant information for tackling problems. This memory is capable of effectively storing and recalling relevant information gathered over time in order to take the next suitable decision in every scenario. UAV obstacle avoidance and navigation also present a similar problem of \emph{partial observability} which requires a notion of memory.
For example, while navigating, a UAV may fly towards a corner. When it is approaching the corner, the depth map might indicate more space in the front when compared to the sides. The lack of temporal information coupled with limited field of vision of the monocular camera makes the UAV to move ahead towards the corner and crash onto the wall. Such scenarios are very common in UAV navigation and hence require a controller which can utilize the relevant past information.
% Partial observability for the video game \emph{Doom} has been explored in \cite{fps}. However, it has not been explored in the context of UAV navigation which presents additional challenges.
% Another scenario where lack of spatial information affects the UAV is when the UAV takes off close to a wall. In this case it only sees the wall in front of it. Since it has not yet seen the environment on other sides, it fails to estimate the relative depth of the wall. 
Our aim is to design a UAV control algorithm which has the capability to combine information obtained over a period of time in order to make better navigation and obstacle avoidance decisions. 


==> related.tex <==
The way to go is to inteliigently use the RGB images obtained from the monocular camera to obtain depth information which will be helpful to plan the UAV trajectory accordingly. 
Recent works leverage deep supervised \cite{punarjay}-\cite{field-monocular} and semi-supervised \cite{semisupdeeplearningdepth} learning techniques for this purpose. Designing a convolutional neural network (CNN) for estimating depth from monocular RGB images is the common thread in these works.
While \cite{punarjay} uses a basic CNN architecture to obtain a depth map from RGB images, 
\cite{fcrn} uses feedback loop architecture (residual networks) for the same. The challenging problem of depth prediction in fast moving UAVs is considered in \cite{fast-monocular}. This work designs a deep neural network to train the predictor on photo-realistic outdoor images generated from a graphic engine. The authors demonstrate that with a little tradeoff in accuracy, this network architecture improvises on the speed of depth prediction (a critical requirement for high-speed UAVs).
The method proposed in \cite{semisupdeeplearningdepth} utilizes monocular as well as stereo images to train a CNN for depth prediction. This way, any shortcomings in alignment of stereo images is covered up by supervised datasets, while the stereo images help in dealing with minimal depth variation information in the datasets. The above works, with the exception of \cite{punarjay} deal with the problem of depth prediction only. Once the depth or range of obstacles is predicted it is imperative to design an algorithm for UAV navigation. 

Varied navigation techniques in conjuction with depth prediction are proposed in \cite{punarjay}, \cite{jmod}-\cite{arxivref2}. \cite{punarjay} proposes a behaviour arbitration scheme to 
obtain the yaw and pitch angles for the UAV to avoid an obstacle and for navigation in general.
Trajectory planning using obstacle bounding boxes and depth estimation is explored in \cite{jmod}.
% However, the navigation cues so obtained are heavily dependent on the training dataset and the simulation environments 
This work designs a CNN architecture that jointly estimates depth and obstacle bounding boxes. The authors then plan trajectories between a start and end point using the RRT-Connect planner. The work \cite{intermediate} proposes two different CNN architectures - one for depth and surface normal estimation and the other for trajectory prediction. Both the CNNs use a 3D cost function for training
and evaluation. \cite{crash-learn} follows an unconventional approach, wherein the authors collect a dataset of UAV crashes. This dataset is classified and feeded to a CNN architecture. Given an image obtained from the monocular camera, the architecture predicts how the UAV should move in the next instant to avoid a crash. 
CAD2RL \cite{cad2rl} proposes a deep reinforcement learning (DRL) method for obstacle avoidance in indoor flight. This work trains a UAV for navigation using only simulated 3D hallway environments. For this, a large number of 3D hallway environments with different lighting, wall textures, furniture placement are generated and the hope is that the UAV can learn to navigate through such hallways even in real-world. Although the works \cite{punarjay}, \cite{jmod}-\cite{cad2rl} can be extended to some specific real-world settings, they require substantial amount of computational and physical resources to generate the huge datasets and train the UAV. \cite{arxivref2} proposes a deep double-Q network with dueling architecture for obstacle avoidance in mobile ground robots.

%"Playing FPS Games with Deep Reinforcement Learning"







